Generalization of the Alpha-Stable Distribution with the Degree of Freedom

A Wright function based framework is proposed to combine and extend several distribution families. The $\alpha$-stable distribution is generalized by adding the degree of freedom parameter. The PDF of this two-sided super distribution family subsumes those of the original $\alpha$-stable, Student's t distributions, as well as the exponential power distribution and the modified Bessel function of the second kind. Its CDF leads to a fractional extension of the Gauss hypergeometric function. The degree of freedom makes possible for valid variance, skewness, and kurtosis, just like Student's t. The original $\alpha$-stable distribution is viewed as having one degree of freedom, that explains why it lacks most of the moments. A skew-Gaussian kernel is derived from the characteristic function of the $\alpha$-stable law, which maximally preserves the law in the new framework. To facilitate such framework, the stable count distribution is generalized as the fractional extension of the generalized gamma distribution. It provides rich subordination capabilities, one of which is the fractional $\chi$ distribution that supplies the needed 'degree of freedom' parameter. Hence, the "new" $\alpha$-stable distribution is a "ratio distribution" of the skew-Gaussian kernel and the fractional $\chi$ distribution. Mathematically, it is a new form of higher transcendental function under the Wright function family. Last, the new univariate symmetric distribution is extended to the multivariate elliptical distribution successfully.

==> yold-gsas-reasoning.tex <==

% -------------------------------------------------------------------------------------
\subsection{Revisit Student-t Distribution}\label{section:student-t}

It is known that a standard t-distribution of degree of freedom \(k\) arises from compounding a standard normal distribution
of unknown variance, with an inverse gamma distribution placed over the variance with parameters
\(\text{IG}(x;\frac{k}{2}, \text{scale}=\frac{k}{2})\). This is where the story began.

The thinking goes like that, if the variance is an IG, then the inverse of variance
is a gamma distribution, which is an SC: \(\scN_{\frac{1}{2}}(z)\). 
Make a similar transition from SC to SV, the inverse of variance becomes inverse of volatility.

Therefore,
\begin{align*}
t_{k}(x) &= D
    \left( 1 + \frac{x^2}{k} \right)^{ -(k+1)/2 },
    &&\text{where} \quad 
    D = \frac{\Gamma(\frac{k+1}{2})}{\sqrt{\pi k} \Gamma(\frac{k}{2})}
\\
    &= C \int_{0}^{\infty} dz \,
        \left( e^{ -z \, {x}^2/4k } \right)
        z^{\frac{k}{2}-1} \scN_{\frac{1}{2}}(z)
    &&\text{where} \quad 
    C = \frac{2^{-k+1} }{ \sqrt{k} \, \Gamma(\frac{k}{2}) } 
\\
    &= C' \int_{0}^{\infty} s \, ds \,
        \left( e^{ -{(sx)}^2/2k } \right)
        s^{k-2} \, V_{1}(s)
    &&\text{where} \quad 
    C' = \frac{2^{(-k+1)/2} }{ \sqrt{k} \, \Gamma(\frac{k}{2}) } 
\end{align*}

The GSV structure, \(V_{1,k}(s) \sim s^{k-2} \, V_{1}(s)\), emerges.
With one more change of variable, we arrive at
\begin{align}
t_{k}(x) &= \int_{0}^{\infty} s \, ds \,
        \mcN(sx) \, V_{1,k}(s)
\end{align}

TODO In fact, t = norm / \(\sqrt{\chi^2_k / k}\)?
\url{https://statproofbook.github.io/P/t-pdf}

The SC formula above is the \(\chi^2\) equivalent, the SV formula is the \(\chi\) equivalent?

% -------------------------------------------------------------------------------------
\subsection{Unifying with Symmetric alpha-Stable Distribution}\label{section:sas-explore}


% -------------------------------------------------------------------------------------
\subsubsection{symmetric stable vs stable count}\label{symmetric-stable-vs-stable-count}

TODO This subsection is just a lot of cut and paste. Need a lot of work.

\begin{align*}
L_\alpha(x) 
    &= \frac{\Gamma(\frac{1}{\alpha}+1)}{\pi} \,
    \int_{0}^{\infty} 
       dt \, \cos(xt) 
       \, \left( \frac{1}{\Gamma(\frac{1}{\alpha}+1)} e^{-t^\alpha} \right)
       \, , \, 0 < \alpha \le 2
\\
    &= \frac{\Gamma(\frac{1}{\alpha}+1)}{\pi} \,
    \int_{0}^{\infty} 
       dt \, \cos(xt) 
       \, \int_{0}^{\infty} \frac{d\nu}{\nu} 
       \left( e^{-t/\nu} \right)
        \mathfrak{N}_\alpha(\nu)
    \, , \, 0 < \alpha \le 1
\\
    &= \frac{\Gamma(\frac{1}{\alpha}+1)}{\pi}
    \, \int_{0}^{\infty} \frac{d\nu}{\nu} 
    \left( \int_{0}^{\infty} dt \, \cos(xt) e^{-t/\nu} \right)
    \scN_\alpha(\nu)
\end{align*}


The inner integral is a Laplace
transform of cosine (See \eqref{eq:int-cosine}). So we arrive at the decomposition

\begin{align}
P_\alpha(x) 
    &= \frac{\Gamma(\frac{1}{\alpha}+1)}{\pi} \,
    \, \int_{0}^{\infty} d\nu
    \left(     \frac{1}{{(\nu x)}^2 + 1} \right)
    \mathfrak{N}_\alpha(\nu)
\\
    &= 
    \, \int_{0}^{\infty} \nu d\nu
    \, \text{Cauchy}(\nu x)
    \, \left( \Gamma\left( \frac{1}{\alpha}+1 \right) \, \nu^{-1} \mathfrak{N}_\alpha(\nu) \right)
\\
    &= 
    \, \int_{0}^{\infty} \nu d\nu
    \, \text{Cauchy}(\nu x)
    \, N_\alpha(\nu; \sigma=1, d=0, p=\alpha)
\\
    &= 
    \, \int_{0}^{\infty} \nu d\nu
    \, P_1(\nu x)
    \, N_\alpha(\nu; \sigma=1, d=0, p=\alpha)
\end{align}

This is similar to the Weibull's Laplace decomposition, except that the
product distribution is changed to the ratio distribution, and the unit
distribution is now Cauchy.

The last statement is saying, \(P_\alpha(x)\) is taking \(P_1(x)\)
with Baysian inference on the ``square root of precision'' by a
generalized stable count.

 -------------------------------------------------------------------------------------


% -------------------------------------------------------------------------------------
\subsubsection{symmetric stable vs stable vol}\label{symmetric-stable-vs-stable-vol}

\begin{align}
P_\alpha(x) 
    &= \frac{ 2 \Gamma(\frac{1}{\alpha}+1)}{\pi} \,
    \int_{0}^{\infty} 
       dt \, \cos(xt) 
       \, \left( \frac{1}{ 2 \Gamma(\frac{1}{\alpha}+1)} e^{-t^\alpha} \right)
       \, , \, 0 \lt \alpha \le 2
\\
    &= \frac{ 2 \Gamma(\frac{1}{\alpha}+1)}{\pi} \,
    \int_{0}^{\infty} 
       dt \, \cos(xt) 
       \, \int_{0}^{\infty} \frac{ds}{s} 
       \left( \frac{1}{\sqrt{2\pi}} e^{-(t/s)^2/2} \right)
        V_\alpha(s)
\\
    &= \frac{ 2 \Gamma(\frac{1}{\alpha}+1)}{\pi} \,
    \, \int_{0}^{\infty} \frac{ds}{s} 
    \left( \frac{1}{\sqrt{2\pi}} \, \int_{0}^{\infty} dt \, \cos(xt) e^{-(t/s)^2/2} \right)
    V_\alpha(s)
\end{align}

The inner integral is a Gaussian
transform of cosine (See \eqref{eq:gauss-cosine}). So we arrive at the decomposition

\begin{align}
P_\alpha(x) 
    &= \frac{ \Gamma(\frac{1}{\alpha}+1)}{\pi} \,
    \, \int_{0}^{\infty} \frac{ds}{s} 
    \left( s \, e^{-(sx)^2/2} \right)
    V_\alpha(s)
\\
    &= 
    \, \int_{0}^{\infty} s ds
    \left( \frac{1}{\sqrt{2\pi}} \, e^{-(sx)^2/2} \right)
    \left( \sqrt{\frac{2}{\pi}} \, \Gamma\left(\frac{1}{\alpha}+1\right) s^{-1} V_\alpha(s) \right)
\\
    &= 
    \, \int_{0}^{\infty} s ds
    \, N(sx)
    \, N_{\frac{\alpha}{2}}(s; \sigma=\frac{1}{\sqrt{2}}, d=0, p=\alpha)
\\ \text{or in Wright fn} \,\,
    &= 
    2 \, \int_{0}^{\infty} ds
    \, N(sx)
    \, W_{-\frac{\alpha}{2},0} \left( -{\left( \sqrt{2} \, s \right)}^{\alpha} \right) 
\end{align}

TODO why not directly link to GSV with d = 0, with a scale parameter \(\alpha^{1/\alpha}\).

This is similar to the Weibull's Rayleigh decomposition, except that the
product distribution is changed to the ratio distribution, and the unit
distribution is now Normal.


\subsubsection{GSaS, finally}\label{section:sas-to-gsas}

Therefore, the generalized symmetric \(\alpha\)-stable distribution is

\begin{align}\label{eq:gsas-def}
L_{\alpha,k}(x) 
    &= 
    \, \int_{0}^{\infty} s ds
    \, \mcN(sx)
    \, \scN_{\frac{\alpha}{2}}(s; \sigma= \sqrt{\frac{k}{2}} \,{\left( \frac{\alpha}{k} \right)}^{1/\alpha}, d=k-1, p=\alpha)
\end{align}
where \(k \ge 1\) is the degree of freedom parameter, as understood in the student-t context.

\begin{itemize}
\item
  This distribution is restored to a rescaled SaS by 
  \(L_{\alpha,1}(x) = P_\alpha(x;\sigma=1/\alpha^{1/\alpha})\).
\item
  This distribution subsumes student-t by \(L_{1,k}(x) = t_k(x)\).
\end{itemize}

Hence, everything in between is generalization. Notice that \(t_k(x)\)
has finite variance for \(k > 2\), and finite kurtosis
for \(k > 4\). We can understand the moment-less \(P_\alpha(x)\) 
as a consequence of being "too low" in the degree of freedom.


==> yold-section-gsv.tex <==


\section{GSV: Generalized Stable Vol Distribution}

This short section defines GSV that will be used extensively later.
The advantage of GSV is that it works well with the normal distribution 
(instead of Laplace distribution) in both the product and ratio distributions.

\(\gsv{x}\) is defined as

\begin{align}\label{eq:pdf-gsv}
\gsv{s} 
    &= \scN_{\frac{\alpha}{2}}\left( s; \sigma=\gsvSigma, d=k-1, p=\alpha \right) 
\end{align} 
where \(s > 0, \alpha \in (0,2], \, k \ge 0\).

The reason for a complicated \(\sigma\) is to achieve three goals. 
First, when \(\alpha = 1\), it is required by the student-t distribution that \(\sigma = 1/\sqrt{2k}\).
See Section \ref{section:student-t} for more discussion.

Second, when \(\alpha \to 2\), GSV is designed to have \(\sigma = 1/\sqrt{2}\) such that
its mean is 1.

Third, as \(k \to \infty\), the mean of the distribution also approaches 1, regardless what \(\alpha\) is.

Additionally, note that \(V_{\alpha,2}(x)\) is a rescaled \(V_\alpha(x)\) whose mean approaches 1
as \(\alpha \to 2\). This is very nice too.

TODO GSV is a generalization of chi distribution?


% -------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------
\subsection{GSV Hankel Integral}
\label{section:gsv-hankel}

Based on GSC's result in Section \ref{section:gsc-hankel}, the Hankel integral of GSV is

\begin{align}
\gsv{x} &= 
    \frac{1}{2\pi i} \int_{H} dt 
    \, C \, {\left( \frac{x}{\sigma} \right)}^{k-2} 
    \, \exp{\left( t- {\left( \frac{x}{\sigma} \right)}^{\alpha} t^{\alpha/2} \right)}
\\ &= 
    \frac{1}{2\pi i} \int_{H} dt \, e^t 
    \, C \, {\left( \frac{x}{\sigma} \right)}^{k-2} 
    \, \exp{\left( - {\left( \frac{x \, t^{1/2}}{\sigma } \right)}^{\alpha}  \right)}
\notag \\
    &= 
    \,  \Gamma\left(\frac{k-1}{2}\right)
    \, 
    \frac{1}{2\pi i} \int_{H} dt 
    \, \left( \frac{e^t }{t^{(k-1)/2}} \right) 
    \, \pdfGG\left( x; a=\frac{\sigma }{ t^{1/2}}, d=k-1, p=\alpha \right)
\notag
\end{align}

TODO: Need to validate these two numerically.

% -------------------------------------------------------------------------------------
\subsection{GSV Moments}
\label{section:gsv-moments}

Based on GSC's moment formula in \eqref{eq:gsc-moment}, it is easy to derive GSV's moments as

\begin{align}\label{eq:gsv-moment}
\E(X^n|\gsv{x}) &= \notag
\E(X^n|N_{\frac{\alpha}{2}}(s; \sigma= \sqrt{\frac{k}{2}} \,{\left( \frac{\alpha}{k} \right)}^{1/\alpha}, 
        d=k-1, p=\alpha))
\\
    &= 
    \sigma^{n} \, 
    \frac{\Gamma(\frac{k-1}{2})} {\Gamma(\frac{k-1}{\alpha})} 
    \frac{\Gamma(\frac{n+k-1}{\alpha})} {\Gamma(\frac{n+k-1}{2})}
    \, , \where
    \sigma= \sqrt{\frac{k}{2}} \,{\left( \frac{\alpha}{k} \right)}^{1/\alpha}
\end{align}

% -------------------------------------------------------------------------------------
\subsubsection{GSV Asymptotic Behavior}
\label{section:gsv-asymptotic}

\textbf{Normal Limit} \quad
As \(\alpha \to 2\), \(\E(X^n|V_{\alpha,k}(x)) \to 1\).
Since both the first moment and second moment are 1, its variance is 0.
It becomes a Dirac delta function. 

\(k \to \infty\), its mean is 1.

\textbf{Student-t Limit} \quad
When \(\alpha = 1\), it is the kernel for student-t in Section \ref{section:student-t}. 
It becomes

\begin{align}
\E(X^n|V_{1,k}(x)) 
    &= {\left( \frac{2}{k} \right)}^{n/2} \,
       \frac{ \Gamma(\frac{n+k}{2}) } { \Gamma(\frac{k}{2}) }
\end{align}

\textbf{SaS Limit}
When \(k = 1\), it is the kernel for SaS in Section \ref{section:sas-explore}. 
It becomes

\begin{align}
\E(X^n|V_{\alpha,1}(x)) 
    &= \left( \frac{{\alpha}^{1/\alpha}}{2^{1/2}} \right)^n \,
    \frac{\Gamma(\frac{n}{\alpha}+1)} {\Gamma(\frac{n}{2}+1)}
\end{align}



% -------------------------------------------------------------------------------------
\subsection{GSV Large k Limit}
\label{section:gsv-large-k}

The moment's formula exhibits elegant linear behavior at large \(k\) when expressed in
\((s-1/2)\) where \(s = 1/\alpha\). The expansion on large \(k\) is first done 
by the Sterling's formula \eqref{eq:gamma-sterling}, then the first two terms of 
\(\log(1+x) = x - x^2/2\) for \(x\) as inverse of \(k\).

\begin{align}\label{eq:gsv-large-k}
\log \E(X^n|V_{\alpha,k}(x)) 
    &= \frac{n^2 - 2n}{2} \left( \frac{ s-1/2 }{k} \right)
\end{align}

\textbf{The Variance at Large \(k\)}

The choice of \(\sigma\) in \eqref{eq:pdf-gsv} produces an elegant property for the variance.
The second moment is predominantly \(m_2 = 1\). And the first moment is 
\(m_1 = \exp(-\frac{s-1/2}{2k})\), which is also very close to 1 
for a reasonable large \(k\) and/or \(s-1/2\) is not too large.  

So the variance is

\begin{align}\label{eq:gsv-var-large-k}
\text{var} = m_2 - m_1^2 
    &= 1- \exp\left( -\frac{s-1/2}{k} \right)
    \approx \frac{s-1/2}{k}
\end{align}

The linear result is elegant. Asymptotically, the variance is just the ratio 
of \((s-1/2)\) and \(k\).

TODO plots here


==> zbad-symbols-nomen.tex <==


%
\nomenclature[D]{\(\pdfGG(x; a, d, p)\)}{The PDF of the generalized gamma distribution} 
%\nomenclature[D]{\(\scN_\alpha(x; \sigma, d, p)\)}{The PDF of the generalized stable count distribution (new)}
%\nomenclature[D]{\(V_{\alpha,k}(x)\)}{The PDF of the generalized stable vol distribution (new)}
%\nomenclature[D]{\({P}_{\alpha,k}(x)\)}{The PDF of the generalized symmetric \(\alpha\)-stable distribution (new)}
%
%\nomenclature[N]{\(\scN_\alpha(\nu)\)}{The PDF of the stable count distribution}
%\nomenclature[N]{\(V_{\alpha}(x)\)}{The PDF of the stable vol distribution}
%\nomenclature[N]{\({L}_{\alpha}(x)\)}{The PDF of the one-sided stable distribution}
%\nomenclature[N]{\({P}_{\alpha}(x)\)}{The PDF of the symmetric \(\alpha\)-stable distribution}
%\nomenclature[N]{\({t}_{k}(x)\)}{The PDF of the student-t distribution}
%
%\nomenclature[O]{\(C\)}{The normalization constant for \(N_\alpha(x; \sigma, d, p)\)}
%\nomenclature[O]{\(\alpha\)}{The Le\'vy stability index}
%\nomenclature[O]{\(d\)}{The degree of freedom parameter in \(N_\alpha(x; \sigma, d, p)\)}
%\nomenclature[O]{\(k\)}{The degree of freedom parameter in \(V_{\alpha,k}(x), P_{\alpha,k}(x), {t}_{k}(x)\)}
%\nomenclature[O]{\(p\)}{The shape parameter in \(N_\alpha(x; \sigma, d, p)\), unless mentioned otherwise}

% -------------------------------------------------------------------------------------
% Really need this section, so that reader can look up. There are just so many symbols.
\subsection{List of Symbols}
\label{section:symbols}
The next list describes the notations and symbols that will be used in this paper:
\printnomenclature

